Robust learning from corrupted EEG with dynamic spatial filtering

Building machine learning models using EEG recorded outside of the laboratory setting requires methods robust to noisy data and randomly missing channels. This need is particularly great when working with sparse EEG montages (1-6 channels), often encountered in consumer-grade or mobile EEG devices. Neither classical machine learning models nor deep neural networks trained end-to-end on EEG are typically designed or tested for robustness to corruption, and especially to randomly missing channels. While some studies have proposed strategies for using data with missing channels, these approaches are not practical when sparse montages are used and computing power is limited (e.g., wearables, cell phones). To tackle this problem, we propose dynamic spatial filtering (DSF), a multi-head attention module that can be plugged in before the first layer of a neural network to handle missing EEG channels by learning to focus on good channels and to ignore bad ones. We tested DSF on public EEG data encompassing ~4,000 recordings with simulated channel corruption and on a private dataset of ~100 at-home recordings of mobile EEG with natural corruption. Our proposed approach achieves the same performance as baseline models when no noise is applied, but outperforms baselines by as much as 29.4% accuracy when significant channel corruption is present. Moreover, DSF outputs are interpretable, making it possible to monitor channel importance in real-time. This approach has the potential to enable the analysis of EEG in challenging settings where channel corruption hampers the reading of brain signals.

==> old_material.tex <==
\subsubsection{Choice of $m_d$}

In \cite{woo2018cbam}, $m_d$ is obtained by max-pooling or average-pooling of Z along the dimensions other than $d$.
To simplify the notation, we describe $m$ below for the case where $d=C$, but this can be extended to the other two dimensions as well.
In the case of average-pooling, we have ($i \in \intset{C}$):

\begin{equation}
    m^{mean}_{C,i} = \frac{1}{T' F} \sum_{j \in \intset{T'}} \sum_{k \in \intset{F}} Z_{i,j,k}
\end{equation}
while for max-pooling, we have:
\begin{equation}
    m^{max}_{C,i} = \max_{j \in \intset{T'}, k \in \intset{F}} Z_{i,j,k}
\end{equation}

The experiments reported in \cite{woo2018cbam} suggest that using a combination of average- and max-pooling helped performance.
The two can be combined by the elementwise summation of the output of $r_{\Omega_d}$ for both $m^{mean}_{d}$ and $m^{max}_{d}$, yielding a modified Eq.~\ref{eq:attention}:
\begin{equation}
    a_{\Phi_d}(Z) = \sigma(r_{\Omega_d}(m^{mean}_d) + r_{\Omega_d}(m^{max}_d))
\end{equation}

We introduce a third way of reducing $Z$ using the frequency-wise covariance matrix $K \in \bbR^{F \times C \times C}$.
We first define the zero-mean embedding $\bar{Z}$: 
\begin{equation}
    \bar{Z}_{i,k} = \frac{1}{T'} \sum_{j \in \intset{T'}} Z_{i,j,k}
\end{equation}
where $i \in \intset{C}$ and $k \in \intset{F}$. We then have:
\begin{equation}
    K_k = \frac{(Z_{i,:,k} - \bar{Z}_{i,k}) (Z_{i,:,k} - \bar{Z}_{i,k})^T}{T'-1}
\end{equation}

Each row $K_{k,i}$ contains the variance of channel $i$ as well as the covariance of channel $i$ with every other channel, for frequency $k$.
We use this information to extract an attention weight for each pair $i,k$ of channel and frequency.
To facilitate the task of the MLP $r_{\Omega_{cov}}$, we copy the diagonal of the covariance matrix and append it as an additional column to the end of the covariance matrix, yielding a matrix $K^* \in \bbR^{F \times C \times (C + 1)}$:
\begin{equation}
    K^* = K \oplus diag(K_{})
\end{equation}
where $\oplus$ is the concatenation operator and $diag$ extracts the diagonal of a square matrix.
This way, the variance information can be readily used by the MLP.
Together, this yields an attention matrix $\alpha_{cov} \in \bbR^{C \times F}$ which can be used as in Eq.~\ref{eq:apply_att}:

\begin{equation}
    \alpha^{cov}_{i,k} = \sigma(r_{\Omega_{cov}}(K^*_{k,i}))
\end{equation}
where $i \in \intset{C}$ and $k \in \intset{F}$.

\subsubsection{Multidimensional attention}

The attention blocks $a_{\Phi_C}$, $a_{\Phi_T}$ and $a_{\Phi_F}$ can be applied in parallel:

\begin{equation}
    Z' = a_{\Phi_C}(Z) \odot (a_{\Phi_T}(Z) \odot (a_{\Phi_F}(Z) \odot Z))
\end{equation}
or, chained sequentially:
\begin{equation}
    Z' = a_{\Phi_C}(Z'^{F,T}) \odot (a_{\Phi_T}(Z'^{F}) \odot (a_{\Phi_F}(Z) \odot Z))
\end{equation}
 where $Z'^{d',d''}$ is the version of $Z$ to which attention has been applied sequentially to dimensions $d'$ and $d''$.
 
 
 \subsubsection{Naive method: interpolation between channels}

Taking inspiration from the interpolation method discussed in Section~\ref{subsec:sota}, we propose a naive way of handling potentially corrupted channels.

In our case, we use MNE-Python's \texttt{interpolate\_bads} method to obtain an interpolation matrix, which we then use to initialize a weight matrix $W \in \bbR ^ {C \times C}$, where the diagonal is 0 ($W_{ij}=0 \quad \text{if}~i=j$)\footnote{We enforce this 0-diagonal constraint by clamping the values of the diagonal to 0 during training.}.

We define the ``interpolation-only'' module $m_{interp}$ as:

\begin{equation}
    m_{interp}(X) = W X
\end{equation}
i.e., the input window $X$ is linearly remapped by replacing each EEG channel by its interpolated version.
The principal limitation of this approach is that given at least one corrupted channel in the input $X$, the interpolated version of all non-corrupted channels will be reconstructed in part from corrupted channels.
This means noise will still be present, however given enough clean channels, the impact of noise might become negligible following the linear transformation.

\subsubsection{Controlling interpolation globally with a single attention weight}

Improving upon the naive interpolation-only approach, it would make sense for the model to decide whether (and to what extent) channels should be replaced by their interpolated version.
For instance, if the channels in a given window are mostly clean, it might be desirable to keep the initial channels; however, if the window is overall corrupted, it might instead be better to replace channels with their interpolated version.

We define the ``scalar-attention'' module $m_{scalar}$ as:

\begin{equation}
    m_{scalar}(X) = \alpha X + (1-\alpha) W X
\end{equation}
where $\alpha \in [0,1]$ is the attention weight predicted by an MLP, i.e. $\alpha_t = \sigma(h_{scalar}(T(X_t)))$ ($\sigma$ is a sigmoid nonlinearity)\hb{Include a $\Theta$ or something like that to indicate h has parameters to be optimized}, $W$ is the same as for the interpolation-only module, and $T$ is a spatial feature extraction transform (e.g., covariance estimation).

While this approach is more flexible, it still suffers from the same limitation as above: there is a chance interpolated channels will be reconstructed from noisy channels.
Moreover, the fact that the attention weight is applied globally, i.e., a single weight applies to all $C$ channels, limits the ability of the module to focus on reconstructing corrupted channels only.

\subsubsection{Controlling interpolation channel-wise with vector attention}
 
The ``vector attention'' module $m_{vector}$ introduces channel-wise attention weights, so that the interpolation can be independently controlled for each channel:
 
 \begin{equation}
     m_{vector}(X) = \text{diag}(\boldsymbol{\alpha}) X + (I - \text{diag}(\boldsymbol{\alpha})) W X
 \end{equation}
where $\boldsymbol{\alpha} \in [0, 1] ^ C$ is again obtained with an MLP, i.e., $\boldsymbol{\alpha}_t=\sigma(h_{vector}(T(X_t))$, and $W$ is as above.

Although more flexible, this version of the attention module still faces the same problem caused by static interpolation weights.

\subsubsection{Dynamic interpolation}

To solve this issue, we build on the previous approach by predicting an attention vector $\boldsymbol{\alpha}$ as before, but this time using a dynamic interpolation matrix $\Omega_t \in \bbR ^ {C \times C}$ obtained with another MLP $h_{d}(X)$:

\begin{equation}
    m_{dyn.interp}(X) = \text{diag}(\boldsymbol{\alpha})X + (I - \text{diag}(\boldsymbol{\alpha})) V(X) X
\end{equation}

In practice, we combine both models $h_{vector}$ and $h_{d}$ into a single MLP $h_{dyn}$ with output $H \in \bbR ^ {C \times C}$, and reshape $H$ into the attention weights $\boldsymbol{\alpha} = \sigma(\text{diag}(H)$ and the interpolation matrix $V_t = (1 - I) \odot \Omega_t$, where $I$ is the identity matrix and $\odot$ is the elementwise matrix product.

\section{Relationship between dynamic interpolation and dynamic spatial filtering approaches}
\label{sec:dsf_derivation}

\hubert{TODO: Reframe this section - DSF was already introduced and so we can focus on the link between dynamic interpolation and DSF. Also, update format of equations.}

In this section, we show that the dynamic interpolation approach described in Appendix~\ref{sec:interp_to_dsf} shares key conceptual connections to dynamic spatial filtering .

The idea is to mimic the interpolation step of a traditional EEG processing pipeline, where a corrupted channel is replaced by a linear combination of the available clean channels.
Therefore, we apply the attention in the following way:

\begin{equation}
    X' = \alpha \odot X + (1 - \alpha) \odot \tilde{X}
\end{equation}
where $X' \in \bbR^{C \times T}$ is the reweighted input window, $\alpha \in \bbR^{C}$ contains a single attention weight per channel, and the interpolated channels $\tilde{X}  \in \bbR^{C \times T}$ is a linear combination of the channels $\tilde{X} = W X$, with $W \in \bbR^{C \times C}$ (each channel is replaced by its interpolated version based on the other $C-1$ channels).

Both $W$ and $\alpha$ are conditioned on the input, through functions $W = \omega(m_K)$ and $\alpha = a(m_K)$ parametrized as, \eg, 2-layer MLPs.
Here, we use the flattened upper half of the covariance matrix of $X$, $m_K \in \bbR^{\frac{C(C+1)}{2}}$, as input to both functions. 
However one could use a different design where the MLPs are directly trained on the input $X$ or some other representation of $X$.

For a specific channel $i$, we can then write:

\begin{equation}
    X'_i = \alpha_i X_i + (1 - \alpha_i) W_i^\top X
\end{equation}
where $X_i$ and $W_i$ are the i-th rows of $X$ and $W$, respectively.
Replacing the first term from the rhs by the dot-product between a vector of zeroes containing the value $\alpha_i$ at position $i$ and the full matrix $X$, we get
\begin{align}
    X'_i =& \begin{bmatrix}
    0 \\
    \vdots \\
    \alpha_i \\
    \vdots \\
    0\\
    \end{bmatrix}^\top X + (1 - \alpha_i) \begin{bmatrix}
    w^i_1\\
    \vdots\\
    w^i_i\\
    \vdots\\
    w^i_C\\
    \end{bmatrix}^\top X
    \\
    =& \begin{bmatrix}
    0 \\
    \vdots \\
    \alpha_i \\
    \vdots \\
    0\\
    \end{bmatrix}^\top X + \begin{bmatrix}
    (1 - \alpha_i) w^i_1\\
    \vdots\\
    (1 - \alpha_i) w^i_i\\
    \vdots\\
    (1 - \alpha_i) w^i_C\\
    \end{bmatrix}^\top X
    =
    \begin{bmatrix}
    (1 - \alpha_i) w^i_1\\
    \vdots\\
    \alpha_i + (1 - \alpha_i) w^i_i\\
    \vdots\\
    (1 - \alpha_i) w^i_C\\
    \end{bmatrix}^\top X
\end{align}

We rewrite for all channels:
 
\begin{equation}
    X' = \begin{bmatrix}
    \alpha_1 + (1 - \alpha_1) w_1^1 & (1 - \alpha_2) w_2^1 & \hdots & (1 - \alpha_C) w_C^1\\
    (1 - \alpha_1) w_1^2 & \alpha_2 + (1 - \alpha_2) w_2^2 & \hdots & (1 - \alpha_C) w_C^2\\
    \vdots & \vdots & \ddots & \vdots\\
    (1 - \alpha_1) w_1^C & (1 - \alpha_2) w_2^C & \hdots & \alpha_C + (1 - \alpha_C) w_C^C\\
    \end{bmatrix} X
\end{equation}
Therefore, this interpolation-based attention module is equivalent to a linear transformation $X' = W_{\mathrm{interp}} X$ where $W_{\mathrm{interp}} \in \bbR^{C \times C}$ is a function of $X$.
Under this interpretation, there could be a single function (instead of the two previous $a$ and $\omega$) that directly outputs $W_{\mathrm{interp}}$ based on $K$.
This is akin to the idea of dynamic spatial filtering, where the weights of a spatial convolutional layer are predicted by a second network conditioned on the input data itself.

\section{Implementation of the matrix logarithm operation}

The matrix logarithm operation is not implemented in PyTorch at the time of writing (v1.6.0).
Therefore, we use different approaches to test out the impact of this operation in our attention modules.

When applying attention on the input layer, we can circumvent the computation of the matrix logarithm in PyTorch as the model does not require backpropagation through the covariance vectorization step.
Therefore, we compute covariance (or Pearson correlation) matrices on the CPU with numpy, and apply scipy's \texttt{linalg.logm} implementation based on a Schur-Pad\'e algorithm to compute the matrix logarithm.\hb{The SVD approach is faster for SPD matrices!}
The result is then passed to our model along with the raw input window $X$.

On the other hand, when applying attention after a temporal convolution layer (i.e., on a filter bank representation), we must be able to backpropagate the error through the matrix logarithm operation.
This means the computation must happen inside the automatic differentiation graph.
A first option consists in using PyTorch's \texttt{symeig} function to perform the operation as formulated in Equation~\ref{eq:matrix_log}.
This implementation based on eigenvalue decomposition is however inefficient on GPU as it requires frequent communication with the CPU. 
Since this is a bottleneck for the training of our models, we implement the matrix logarithm of a square matrix $A$ using its Taylor expansion \cite{dieci1996computational}:

\begin{equation}
    \log(A) = \sum_{k=1}^{\infty}(-1)^{k+1}\frac{(A-I)^{k}}{k}
\end{equation}
The series will converge if $\left\Vert A-I \right\Vert < 1$.
Therefore, to improve convergence, we first normalize $A$ by its Frobenius norm, i.e., $\hat{A}=\frac{A}{\left\Vert A \right\Vert_F}$.\footnote{We found empirically that dividing the norm by 2 before normalizing further helped convergence.}
After evaluating the series, the impact of the normalization on the final answer can be reversed by adding back the normalization factor:

\begin{equation}
    \log(A) = \log(\hat{A}) + \log(\left\Vert A \right\Vert_F) I
\end{equation}

The accuracy of the Taylor approximation is controlled by the number of terms $n$ to be used.
While higher $n$ will produce a better estimate, they also require more matrix multiplications, lengthening both the forward and backward propagation graphs.
To test the impact of $n$ on the quality of the estimate, we compared scipy's implementation to our Taylor approximation on TUAB data.
Results are presented in Fig.~\ref{fig:logm_taylor}.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{logm_taylor.png}
    \caption{Impact of the number of Taylor series terms used in the matrix logarithm approximation on the quality of the estimate. For each $n$, we compare the matrix logarithm estimate to the value of scipy's \texttt{linalg.logm} on 1,000 random windows sampled from TUAB's eval set (6 channels) and transformed into covariance or correlation matrices. The relative error is computed as $\frac{\left\Vert \text{logm}(\Sigma) - \text{logm}_{Taylor}(\Sigma) \right\Vert_2}{\left\Vert \text{logm}(\Sigma) \right\Vert_2}$. Shaded areas indicate standard deviation. Under clean conditions, it takes at least 20 iterations to obtain an estimate with less than 10\% error on covariance matrices. When additive white noise is added, the quality of the approximation decreases, and a relative error below 10\% is not reached within 100 terms. On correlation matrices, the estimate obtained is not affected by noise, and takes above 30 iterations to reach 10\% relative error.}
    \label{fig:logm_taylor}
\end{figure}
% Results from comparing_logm_and_logm_taylor.ipynb

Overall, the high number of terms required to obtain a good estimate, especially under noisy conditions, indicates that this approach is not efficient.
A native PyTorch implementation of the matrix logarithm using a similar algorithm to scipy's might be the way forward.
Nonetheless, the operation being more robust on correlation matrices, it might be easier to use when the selected spatial transformation is not covariance.

\section{Grid search on number of temporal and spatial filters in ShallowNet}

To motivate the choice of architecture hyperparameters for the ShallowNet model, we performed a grid search over different numbers of temporal and spatial filters in the first two convolutional layers.
The results are presented in Fig.~\ref{fig:n_filters_grid_search}.

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{n_filters_grid_search.png}
    \caption{Grid search on number of temporal and spatial filters in ShallowNet. Models were trained on the development set of TUAB, split subject-wise into train, validation and test sets (70, 10 and 20\% of the subjects, respectively). We used a montage with 6 channels (Fp1, Fp2, A1, A2, Cz and Fz). Results are the average of two random initializations. 
    The number of filters suggested in \cite{schirrmeister2017deep} (i.e., 40 filters for both) yields the second highest result, suggesting this is indeed an optimal choice. However, some configurations with fewer filters perform similarly, for instance 10 temporal filters and 40 spatial filters.}
    \label{fig:n_filters_grid_search}
\end{figure}
% Results: multirun/2020-10-06/17-17-35 (1263-1334)
% Code:
% # Testing impact of n_spatial_filters and n_time_filters
% filters_df = results_df[['model.emb.n_time_filters', 'model.emb.n_spatial_filters', 'test_bal_acc']]
% filters_df = filters_df.groupby(['model.emb.n_time_filters', 'model.emb.n_spatial_filters']).mean().reset_index()
% filters_bal_acc = filters_df[['model.emb.n_time_filters', 'model.emb.n_spatial_filters', 'test_bal_acc']].pivot(
%     index='model.emb.n_time_filters', columns='model.emb.n_spatial_filters', values='test_bal_acc')
% fig, ax = plt.subplots(figsize=(5, 4))
% ax = sns.heatmap(filters_bal_acc, annot=True, fmt='0.3f', cbar_kws={'label': 'test bal acc'}, ax=ax)
% ax.set_xlabel('Number of spatial filters')
% ax.set_ylabel('Number of temporal filters')

While the number of filters suggested in \cite{schirrmeister2017deep} (i.e., 40 filters for both) indeed yields one of the highest performance, some configurations with fewer filters perform similarly.

\section{Impact of number of EEG channels on performance under noisy conditions}
\label{sec:impact_of_noise}

We explored the effect of varying noise level for different numbers of input EEG channels. 
Results are presented in Fig.~\ref{fig:impact_n_channels_under_noise}, with the montages described in Table~\ref{tab:montages}.
Although using all available channels yielded the highest performance, very similar performance could be obtained with subsampled montages.
Importantly, channel corruption has a higher detrimental effect on sparser montages.

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{impact_noise_n_channels.png}
    \caption{Pathology detection performance for different numbers of input EEG channels and under varying levels of noise. ShallowNet was trained on TUAB with one up to 21 input EEG channels, while the probability of randomly corrupting channels with white noise varied from 0 to 1. White noise had  standard deviation $\sigma \sim\mathcal{U}(20,50)$~$\mu$V and strength $\eta \sim\mathcal{U}(0.5,1)$. (Average of two random initializations; on train set) The higher the number of available channels is, the less performance was affected by missing channels. Close to full montage performance was reached with only a subset of the electrodes (\eg, 10 or 6).}
    \label{fig:impact_n_channels_under_noise}
\end{figure}

\begin{table}[]
\begin{tabular}{cl}
\# channels & Channels                                                     \\
\hline
1                  & Cz                                                           \\
2                  & T3, T4                                                       \\
4                  & Fp1, Fp2, T3, T4                                             \\
6                  & Fp1, Fp2, T3, T4, Cz, Fz                                     \\
10                 & Fp1, Fp2, T3, T5, T4, T6, Cz, Fz, O1, O2                     \\
15                 & Fp1, Fp2, F3, F4, T3, T5, T4, T6, Cz, C3, C4, Fz, Pz, O1, O2 \\
21                 & All                                                         
\end{tabular}
\caption{Subsampled montages used in TUAB experiments.}
\label{tab:montages}
\end{table}

\section{Impact of number of virtual channels on performance}
\label{sec:impact_n_virtual_channels}

The number of virtual channels (i.e., attention heads) $C'$ in the DSF module is a hyperparameter that can be optimized.
We performed a search over different values of $C'$ on the TUAB dataset using a DSF module and the data augmentation denoising approach.
Performance evaluation over different noise configurations is presented in Fig.~\ref{fig:impact_n_virtual_channels}.

While setting $C'=C$ did not lead to the best performance, sing a few additional virtual channels improved robustness to noise.
Above 9, however, performance decreased again.
Interestingly, using only 4 virtual channels also yielded better results than $C'=C$. 
This suggests a small amount of redundancy or conversely some dimensionality reduction might help the network cope with noise.

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{impact_n_virtual_channels.png}
    \caption{Pathology detection performance for different numbers of DSF virtual channels $C'$, under increasing levels of noise. ShallowNets were trained on TUAB with 6 input EEG channels but 4 to 12 virtual channels, under additive white noise data augmentation of strength 0 to 1. Results obtained with two different random initializations and three random splits. Creating more virtual channels than input channels seems to improve robustness to noise, although above 9 virtual channels the performance starts to degrade again.}
    \label{fig:impact_n_virtual_channels}
\end{figure}
% /storage/store2/work/hjacobba/experiments/perf_under_noise/223/results.csv

\section{Impact of common average referencing on downstream performance}

In our experiments on TUAB we created reduced montages by subsampling the available electrodes.
However, since the original data was originally preprocessed with a common average reference (CAR), one could argue that the subsampled montages still contain information that would not be accessible if only these subsampled channels had been initially recorded.
From this perspective, the downsampled montages should therefore be re-referenced to replicate realistic sparse montage conditions.

We tested the impact of applying CAR on the subsampled montages in Fig.~\ref{fig:impact_car_ref}.
Re-applying CAR did not hamper performance when all channels were available or no additional corruption was applied, however it did negatively impact the model trained on 6 channels and noise, which lost about 2\% balanced accuracy.
This difference suggests that sparser models benefit more strongly from the full-montage CAR, and therefore that a more realistic benchmark indeed requires re-referencing the data after the montage downsampling step.

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{impact_car_ref.png}
    \caption{Pathology detection performance with and without additional common average re-referencing. ShallowNet was trained on TUAB with 6 or 21 input EEG channels, with white noise corruption probability of 0 or 0.5, and either the original reference, or a new CAR reference. Results obtained with two different random initializations. While re-referencing did not negatively impact performance when 21 channels were used or no corruption was applied, it did negatively impact performance of the model trained on 6-channel, noisy data.}
    \label{fig:impact_car_ref}
\end{figure}
% Results: multirun/2020-10-08/00-29-36 + multirun/2020-10-08/16-12-19 (1361-1368 + 1369-1376)
% Code:
% def make_model_name(row):
%     n_transforms, n_channels = row['n_transforms'], row['n_channels']
%     transform = 'Original reference' if n_transforms == 1 else 'Rereferenced'
%     return f'{n_channels} channels ({transform})'

% results_df['model'] = results_df.apply(make_model_name, axis=1) 

% fig, ax = plt.subplots(figsize=(4, 3))
% g = sns.stripplot(
%     data=results_df, y='test_bal_acc', x='transforms.0.p', hue='model',
%     palette='colorblind', dodge=True, ax=ax, 
%     hue_order=[
%         '6 channels (Original reference)',
%         '6 channels (Rereferenced)',
%         '21 channels (Original reference)',
%         '21 channels (Rereferenced)',
%     ])
% ax.set_xlabel('Corruption probability');
% ax.set_ylabel('Test bal acc');

\section{Performance of Riemann method trained under varying levels of noise}

The performance of the Riemannian geometry baseline is presented in Fig.~\ref{fig:impact_noise_riemann_tuh}.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{impact_noise_n_channels_lineplot_riemann_tuh.png}
    \caption{Pathology detection performance for different numbers of input EEG channels and under varying levels of noise for the Riemannian geometry baseline. ShallowNet was trained on TUAB with one up to 21 input EEG channels, while the probability of randomly corrupting channels with white noise varied from 0 to 1. White noise had standard deviation $\sigma \sim\mathcal{U}(20,50)$~$\mu$V and strength $\eta \sim\mathcal{U}(0.5,1)$ (average of two random initializations times two random splits; on dev set). The higher the number of available channels is, the less performance was affected by missing channels. Close to full montage performance was reached with only a subset of the electrodes (\eg, 10 or 6).}
    \label{fig:impact_noise_riemann_tuh}
\end{figure}
% Results: 
%   multirun/2020-10-21/17-44-47 (fb_riemann_pathology_detection/95-164)
%   multirun/2020-10-22/16-37-19 (fb_riemann_pathology_detection/165-234)
% Code:
% ax = sns.lineplot(
%     data=results_df, x='noise.p', y='test_acc', hue='n_channels', 
%     palette='colorblind', style='n_channels', markers=True, dashes=True, ci=None,
%     alpha=0.7, ms=8)
% ax.set_xlabel('Channel corruption probability')
% ax.set_ylabel('Test accuracy')
% ax.legend(title='Number of\nchannels')

\section{Related work}
Noise robust speech processing:
- \cite{seltzer2013investigation}: 2013, speech recognition, "noise-aware training" where the network also receives as input an estimate of the noise level + dropout helped improve perf by 7.5\% over SOTA
- \cite{serdyuk2016invariant}: 2016, speech recognition, noise invariance, two heads (1) speech recognition classifier and (2) domain discriminator to distinguish between different types of noise (simulated) with gradient reversal
- \cite{liang2018learning,salazar2018invariant}: "invariant representation learning", penalizes the distance between the internal representation of clean and noisy examples,

With deep beamforming:
- \cite{wittevrongel2017spatiotemporal}: spatiotemporal beamforming for EEG BCIs
- \cite{li2016neural}: neural adaptive beamforming, 2-channel speech recognition, a "filter prediction" subnetwork generates temporal filters for each of the 2 input signals, improvement over simpler approaches and more efficient
- \cite{xiao2016deep}: beamforming, multiple channel speech recognition, a branch finds beamforming filters (per frequency bin and channel - essentially one spatial filter per frequency bin) which are then applied, input to beamformer network is GCC (generalized cross-correlation) but they talk about using covariance matrices in conclusion
- \cite{xiao2016beamforming}: follow-up from previous, but using spatial covariance matrices as input, minor improvement over GCC
- \cite{meng2017deep}: adaptive beamforming using LSTM
- \cite{he2020spatial}: fixed weight beamforming with many "look directions" (i.e., spatial filters), then spatial attention [0, 1] to decide which filters to focus on
